SepLLM: Accelerate Large Language Models by Compressing One Segment into One Separator

Large Language Models (LLMs) have exhibited exceptional performance across a spectrum of natural language processing tasks. However, their substantial sizes pose considerable challenges, particularly in computational demands and inference speed, due to their quadratic complexity. In this work, we have identified a key pattern: certain seemingly meaningless separator tokens (i.e., punctuations) contribute disproportionately to attention scores compared to semantically meaningful tokens. This observation suggests that information of the segments between these separator tokens can be effectively condensed into the separator tokens themselves without significant information loss. Guided by this insight, we introduce SepLLM, a plug-and-play framework that accelerates inference by compressing these segments and eliminating redundant tokens. Additionally, we implement efficient kernels for training acceleration. Experimental results across training-free, training-from-scratch, and post-training settings demonstrate SepLLM's effectiveness. Notably, using the Llama-3-8B backbone, SepLLM achieves over 50% reduction in KV cache on the GSM8K-CoT benchmark while maintaining comparable performance. Furthermore, in streaming settings, SepLLM effectively processes sequences of up to 4 million tokens or more while maintaining consistent language modeling capabilities.

==> spjvjgywrcgsfttxpzygsccdcktfvmxn_arXiv/latex/conclude.tex <==
\section{Native Sparse Attention and Language Modeling}
SepLLM essentially models sparsity based on the natural semantic distribution of natural language. During the pre-training phase, SepLLM intentionally compresses segment information into the separator used to divide the segment. This approach closely aligns with the semantic distribution of natural language because the separator itself provides a division and summary of the current segment. The segments separated out are inherently semantically coherent, forming self-contained semantic units. Therefore, \textbf{we can view SepLLM as a native sparse attention mechanism inherent to natural language itself}. Moreover, SepLLM is suitable to replace StreamingLLM (which only statically focuses on important positions and is overly sparse) as the fundamental baseline model for sparse attention mechanisms in LLMs.





\section{Concluding Remarks}
\label{sec:conclusion}

In this paper, we focus on efficient neural architecture modification to address the computational and storage challenges in LLMs, especially when processing long inputs. From the visualization of attention maps, we find that certain separator tokens consistently contribute high attention scores. Inspired by this, we propose SepLLM, a new language modeling perspective and a sparse attention mechanism,  focusing attention computation on Initial, Neighboring, and Separator Tokens. To achieve wall-clock time acceleration, we also implement hardware-efficient kernels. Our training-free studies suggest these separators effectively compress segment information, enabling efficient information retrieval. Unlike previous training-free methods, SepLLM can be incorporated into the training phase, \eg, training-from-scratch or post-training, thus reducing disparities between training and inference. Extensive experiments across various settings have demonstrated SepLLM's practical effectiveness. 



==> spjvjgywrcgsfttxpzygsccdcktfvmxn_arXiv/latex/exp.tex <==
\section{Experiments and Results}
\label{sec:experiments}

\subsection{Experimental Settings}
\label{sec:cmn_setup}
We evaluate our proposed~\model~on the following tasks, \ie, training-free, training-from-scratch, post-training, and streaming applications. 




\vspace{-0.1in}
\paragraph{Model.} Two popular model families, \ie, Pythia \citep{biderman2023pythia} and Llama-3 \citep{dubey2024llama}, are employed for evaluation.
Specifically, Pythia-160m-deduped is used as the backbone in the training-from-scratch tasks since the model, data, configurations, and checkpoints are all open-source and the training results are reproducible.
As for post-training settings, we take Pythia-1.4B-deduped as our backbone model. 
Even though Llama-3 exhibits powerful performance on various downstream tasks, the training experimental details are not available. 
Therefore, we only use Llama-3 for training-free and streaming tasks. 

 
\vspace{-0.1in}
\paragraph{Training Datasets.} In the training-from-scratch and post-training tasks, the deduplicated Pile \citep{gao2020pile} is utilized for training, which contains about 207B tokens. And all other configurations are the same as the corresponding settings as Pythia \citep{biderman2023pythia}. Specifically, the training epoch is set to 1.5 epoch (143000 steps with the global batch size as 1024), which means about 300B tokens in total are utilized for training from scratch, which is identical to Pythia~\cite{biderman2023pythia}.

\paragraph{Parameter Setting.} The official 93,000-step checkpoint of Pythia-1.4B-deduped model 
is used to conduct post-training, which corresponds to just completing one epoch of training on the 
deduped Pile dataset~\cite{gao2020pile}.\! And [``.", ``,", ``?", ``!", ``;", ``:", `` ", ``\textbackslash t", ``\textbackslash n"] are separator tokens used for all evaluations.
More specific experimental settings are introduced in the respective experiment sections.







\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{8pt}
\setlength\extrarowheight{2.5pt}
\begin{tabular}{l|ccc|cccccc}
& \multicolumn{3}{c|}{GSM8K-CoT}  & \multicolumn{5}{c}{MMLU} \\               
& flexible  & strict    & \rKV~(\%)     & humanities     & stem     & social     & other       & Overall        & \rKV~(\%)   \\ \shline  
Vanilla                                 & 77.79    & 77.26    & 100.00         & 60.49        & 56.61    & 76.50        & 72.19        & 65.72         & 100.00  \\
StrmLLM (\pn=380)       & 70.89    & 71.42    & 47.54         & 57.73        & 54.46    & 74.39        & 70.13        & 63.39         & 52.50   \\
StrmLLM (\pn=256)       & 69.67    & 68.61    & 26.00         & 62.10        & 54.49    & 73.06        & 69.78        & 62.10         &  37.73  \\\rowcolor{Gray}
SepLLM (\pn=256)        & 77.18    & 77.18    & 47.36         & 57.66        & 56.49    & 76.21        & 72.19        & 64.68         & 44.61   \\
\end{tabular}
\vspace{-0.1in}
\caption{Evaluation results and average \textit{runtime} KV cache usage for training-free experiments on GSM8K-CoT 8-shots and MMLU 5-shots. For~\model~and StreamingLLM, three initial tokens' KV are kept for this experiment. \rKV~(\%) here represents the ratio of KV usage at \textit{runtime} for the respective method compared to Vanilla. See more results in Appendices~\ref{sec:appendix_fix_int} and Table~\ref{tab:fixed_sepllm}.}
\label{tab:training_free}
\end{table*}

\subsection{Training-Free}
We evaluate the proposed~\model~architecture in the training-free tasks based on the popular Llama-3-8B-Instruct model~\citep{dubey2024llama}.
\paragraph{Benchmarks.} The representative and commonly-used  GSM8K-CoT \citep{cobbe2021training} and MMLU~\citep{hendrycks2021measuring}) are adopted. 
{{GSM8K-CoT}}~\cite{cobbe2021training}  tests a model's ability to solve mathematical problems by evaluating its reasoning and step-by-step problem-solving skills. {CoT}~\cite{wei2022chain} means the ability to simulate a reasoning process by breaking down complex problems into a series of logical steps. And the default 8 shots are adopted.
{{MMLU}}~\cite{hendrycks2021measuring} assesses a model's general knowledge and reasoning ability across a wide range of subjects, such as history, science, mathematics and so on.
The commonly-used 5-shot setting is used for {MMLU}.
\begin{table*}[ht]
\small
\setlength{\tabcolsep}{7pt}
\setlength\extrarowheight{2pt}
\centering
\begin{tabular}{l|ccccccc|cc}
Method                             & ARC-c  & ARC-e  & LBD-ppl  & LBD-acc & LogiQA & PIQA   & SciQ   & Atten. (\%) & \rKV~(\%) \\ \shline
Vanilla                            & 20.14  & 46.80  & 34.83    & 33.28   & 23.81  & 62.84  & 81.50  & 100.00   & 100.00   \\
StrmLLM(\pn=64)    & 20.65  & 47.39  & 44.03    & 26.74   & 21.97  & 63.82  & 75.80  & 16.58    & 15.28    \\\rowcolor{Gray}
\model (\pn=64)    & 19.62  & 46.46  & 40.08    & 28.97   & 26.42  & 63.82  & 80.10  & 25.83    & 25.40    \\\rowcolor{Gray}
\model (\pn=128)   & 19.97  & 47.35  & 30.16    & 33.18   & 22.73  & 64.64  & 82.60  & 35.64    & 32.27    \\\rowcolor{Gray}
\model (\pn=64,H)  & 20.73  & 48.44  & 36.54    & 30.45   & 25.35  & 64.36  & 80.60  & 32.01    & 31.58    \\\rowcolor{Gray}
\model(\pn=64,H/T) & 21.42  & 47.26  & 33.41    & 32.80   & 22.73  & 63.98  & 81.20  & 38.18    & 37.75   
\end{tabular}
\vspace{-0.1in}
\caption{The performance of downstream tasks and the average \textit{runtime} KV cache usage in the training-from-scratch setting.}
\label{tab:trn_downstream}
\end{table*}












\paragraph{Results.}The experimental results for training-free are shown in Table~\ref{tab:training_free}. ``Vanilla" represents the original Llama-3 model with full attention, while ``StrmLLM" represents StreamingLLM~\cite{xiao2024efficient}.~\pn~means the number of KV for Neighboring Tokens we retain. 
For~\model, all the KV for Separator Tokens are kept and for the setting \textit{SepLLM (\textbf{n}=256)}, we find that~\model~exhibits comparable performance in both multi-step mathematical CoT task and multidisciplinary knowledge reasoning tasks, when compared to the full-attention Llama-3.~\model~achieves this using only 47.36\% of the KV utilized by the original Llama-3 for reasoning, indicating~\model's capability of modeling both the contexts requiring multi-step logical analysis and those involving multi-domain knowledge reasoning while retaining only 50\% original KV.



\textit{StrmLLM (\textbf{n}=256)} setting corresponds to removing all separators' KV from \textit{~\model~(\textbf{n}=256)} setting, except for those in Neighboring and Initial tokens. We observe a noticeable decrease in both mathematical analysis and multidisciplinary knowledge reasoning abilities for \textit{StrmLLM (\textbf{n}=256)}. \textit{StrmLLM (\textbf{n}=256)} utilizes only 26.00\% and 37.73\% of the KV for the GSM8K and MMLU tasks, respectively, which are less than \textit{~\model~(\textbf{n}=256)} (47.36\% and 44.61\% respectively). Consequently, we increase the~\pn~of \textit{StrmLLM} to 380, aligning the kept KV on GSM8K to be equal to \textit{~\model~(\textbf{n}=256)} (approximately 47\%, while on MMLU task, \textit{StrmLLM (\textbf{n}=380)} retains 52.5\% of the KV, significantly higher than \textit{~\model~(\textbf{n}=256)}). This leads to improved performance compared to \textit{StrmLLM (\textbf{n}=256)}. However, it still remains lower than the full-attention Llama-3 and \textit{~\model~(\textbf{n}=256)}. This indicates that the KV of separators indeed encapsulates information contained within their respective segments, and removing them significantly impacts the Transformer's understanding and reasoning abilities.








































\begin{figure}[t]
    \centering
    \vspace{-2mm}
    \subfigure[Loss \wrt~steps]{ \includegraphics[width=0.47\columnwidth]{fig/training_loss_SepLLM_v5.pdf}\label{fig:training_loss_a}}
    \subfigure[Loss Ratio \wrt~FLOPs]{\includegraphics[width=0.47\columnwidth]{fig/TFLOPs_r_SepLLM_v5.pdf}\label{fig:training_loss_b}}
    \vspace{-0.16in}
    \caption{Training loss curves for training from scratch. \ref{fig:training_loss_b} shows the ratios of the loss values of different methods to that of Vanilla with respect to FLOPs.}
    \label{fig:training_loss}
    \vspace{-0.15in}
\end{figure}

\subsection{Training from Scratch}
\label{sec:trn_scratch}

We train the original Pythia-160m-deduped model as well as the Pythia-160m-deduped model modified with the~\model~(and StreamingLLM) architecture on the Pile dataset for 143,000 steps using a global batch size of 1024 (involving approximately 300B tokens in total for training). All training configurations are consistent with Pythia~\citep{biderman2023pythia} (see Section~\ref{sec:cmn_setup}). And following Pythia~\citep{biderman2023pythia}, we conduct tests on the following downstream tasks: ARC-Challenge and ARC-Easy \citep{clark2018think}, LAMBADA \citep{paperno-etal-2016-lambada} (for Perplexity and Accuracy), LogiQA~\citep{liu2020logiqachallengedatasetmachine}, PIQA~\citep{bisk2020piqa},  SciQA~\citep{welbl2017crowdsourcing}. From the loss curves depicted in Figure~\ref{fig:training_loss} and the downstream performance in Table~\ref{tab:trn_downstream}, we draw the following analysis.
\paragraph{Neighboring Token Benefits.} Based on the experiments with the settings \textit{SepLLM (\textbf{n}=64)} and \textit{SepLLM (\textbf{n}=128)}, we find that during training, increasing Neighboring Tokens (\pn) leads to a faster decrease in the training loss curve (Figure~\ref{fig:training_loss}).  Furthermore, models trained with larger~\pn~exhibit stronger performance in downstream tasks (Table~\ref{tab:trn_downstream}). This highlights the important role of neighboring tokens in contextual language modeling and downstream task inference.    
\paragraph{Hybrid Layer Benefits.}  We find that employing a certain hybrid architecture is beneficial to both the training loss and the performance on downstream tasks. For instance, by modifying only the first self-attention layer to full attention in the experiment corresponding to \textit{SepLLM (\textbf{n}=64)} (denoted as \textit{SepLLM (\textbf{n}=64,H)}), there is a moderate optimization in both the training process and downstream tasks. If both the first and last attention layers are changed to full attention (denoted as \textit{SepLLM (\textbf{n}=64,H/T)}), this optimization becomes more pronounced. For example, LAMBADA perplexity decreases from 40.08 for \textit{SepLLM (\textbf{n}=64)} to 36.54 for \textit{SepLLM (\textbf{n}=64,H)}  and 33.41 for \textit{SepLLM (\textbf{n}=64,H/T)}.
\paragraph{Separators' Role.} The experiment with the setting \textit{StrmLLM (\textbf{n}=64)} corresponds to \textit{SepLLM (\textbf{n}=64)}, but does not consider separators other than those in Neighboring and Initial tokens. We observe a significant slowdown in the training loss decrease for \textit{StrmLLM (\textbf{n}=64)}, and its performance deteriorates across various downstream tasks. This indicates that the KV corresponding to separators indeed contain information about the segments they belong to, which are beneficial to predicting subsequent tokens.

\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{l|c|cccc|c}
Arch.      & StrmLLM & \multicolumn{4}{c|}{SepLLM}  & Vanilla                                                                                                      \\ 
Setting           & \pn=64    & \multicolumn{1}{c}{\pn=64}  & \multicolumn{1}{c}{\pn=128} & \multicolumn{1}{c}{\pn=64,H} & \multicolumn{1}{c|}{\pn=64,H/T} & full \\ \shline
FLOPs (\%)   & 70.11   & \multicolumn{1}{c}{71.77} & \multicolumn{1}{c}{72.58} & \multicolumn{1}{c}{72.83}  & \multicolumn{1}{c|}{73.90}    & 100.0        \\ 
Atten. (\%) & 6.43    & \multicolumn{1}{c}{17.21} & \multicolumn{1}{c}{22.48} & \multicolumn{1}{c}{24.11}  & \multicolumn{1}{c|}{31.01}    & 100.0   \\
\end{tabular}
\vspace{-2mm}
\caption{The comparison of FLOPs and Attention Map Ratios.}
\label{tab:tab_flops}
\vspace{-3.5mm}
\end{table}


We also investigate the FLOPs and Attention Map Ratio (indicating the proportion of '1's in the lower triangle of the attention mask) required by the different architectures when trained on the same input data. As shown in Table~\ref{tab:tab_flops}, We find that~\model~can significantly reduce FLOPs by approximately 30\%. After plotting the loss ratios between~\model~and Vanilla under the same FLOPs (see Figure~\ref{fig:training_loss_b}), we observe that SepLLM has lower loss than Vanilla. This indicates that our~\model~architecture at least has a comparable ability to extract useful information from the dataset during training as Vanilla. Besides, the detailed wall-clock time per iteration and the wall-clock time speedups are illustrated in Appendix~\ref{app:training_acc} and Figure~\ref{fig:TFLOPs}.





                     




\subsection{Post-Training}
Since training from scratch is time-consuming, we also conduct post-training experiments using 93000-step Pythia-1.4B-deduped checkpoint officially released by Pythia (see Section~\ref{sec:cmn_setup} for details). Figure~\ref{fig:post_training_loss} displays the loss curves for post-training, where \textit{SepLLM (\textbf{n}=64, larger lr)} denotes we employ an entire cosine learning rate scheduler (including a warm-up process starting from 0) identical to that of original Pythia-1.4B-deduped from step 0. \textit{SepLLM (\textbf{n}=64)} and \textit{SepLLM (\textbf{n}=128)} utilize a cosine learning rate scheduler that continues to decay from the 93000th step. From Figure~\ref{fig:post_training_loss}, it is evident that increasing~\pn~and appropriately raising the learning rate both facilitate the decrease in loss. Moreover, this also illustrates that~\model~can achieve a swift transformation from a full-attention LLM checkpoint to a model that aligns with the requirements of the~\model~architecture's embedding distribution through post-training.

\begin{figure}[t]
    \vspace{-0.25mm}
    \centering
    \includegraphics[width=0.75\linewidth]{fig/post_train_SepLLM_v5.pdf}
    \vspace{-0.2in}
    \caption{Training loss curves for the post-training setting.}
    \label{fig:post_training_loss}
    \vspace{-0.2mm}
\end{figure}

\subsection{Streaming Applications}
\label{sec:stream_app_eval}
\model~can also adapt well to streaming applications, where infinite-length interactions may occur. Here, we follow StreamingLLM~\cite{xiao2024efficient} to validate the scenarios of infinite-length interactions using our \textit{Tailored Streaming Design} on the commonly used PG19 dataset~\cite{raecompressive2019}, which comprises 100 extensive literary works. The results are shown in Table~\ref{tab:stream_pg19}. We can observe that for the same KV cache capacity \textbf{\textit{c}}, the average perplexity of predicting the next token through~\model~remains consistently lower than that of streamingLLM~\cite{xiao2024efficient} within the range from 1M to 4M input length. This once again verifies the ability of KV corresponding to separators to compress segment information and their impact on predicting the probability distribution of the next token. 

\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{3.25pt}
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{l|ccccccc}
\textbf{PG19} & 1M   & 1.5M & 2M   & 2.5M & 3M   & 3.5M & 4M   \\ \shline
StrmLLM        & 39.5 & 38.2 & 38.3 & 37.6 & 36.4 & 35.8 & 36.1 \\ \rowcolor{Gray}
SepLLM (\textbf{\textit{s}}=32)          & 37.7 & 36.6 & 36.6 & 36.0 & 34.9 & 34.2 & 34.5 \\ \rowcolor{Gray}
SepLLM (\textbf{\textit{s}}=64)          & 37.1 & 36.0 & 36.1 & 35.4 & 34.3 & 33.7 & 33.9 \\ 
\end{tabular}
\vspace{-0.1in}
\caption{The perplexity comparison on the PG19 test set~\cite{raecompressive2019}. For fair evaluation, we keep the entire KV cache capacity \textit{\textbf{c}} as 324 and Initial Cache capacity \textit{\textbf{a}} as 4 for both StreamingLLM and~\model. \textit{\textbf{w}}=224, \textbf{\textit{s}}=32/64 for~\model. \label{tab:stream_pg19}}
\vspace{-5.5mm}
\end{table}


We also test the end-to-end inference time of Vanilla, StreamingLLM and our SepLLM on PG19~\cite{raecompressive2019} test set based on LlaMA-3-8B~\cite{dubey2024llama}. Based on the aforementioned settings, we used these LLMs to generate 20K and 64K tokens to evaluate their total inference time (wall-clock time), average perplexity, and average runtime KV cache usage. For both SepLLM and StreamingLLM, the maximum whole KV cache capacity was set to 800 (\ie, \textbf{\textit{c}}=800), and the Initial Cache capacity was set to 4 (\ie, \textbf{\textit{a}}=4). For SepLLM, we additionally set \textbf{\textit{s}}=64 and \textbf{\textit{w}}=256. The results are shown in Table~\ref{tab:infer_time}.
\begin{table}[t]
    \centering
    \small
    \setlength{\tabcolsep}{7pt}
    \renewcommand{\arraystretch}{1.2}
    \begin{tabular}{l|l|cccc}
        Length & Methods & $\textit{\textbf{c}}$ & \rKV & ppl & time (s) \\ \shline
        \multirow{3}{*}{20K} & Vanilla & 20K & 10K & 302.6 & 523.8 \\ 
        ~ & StrmLLM & 800 & 800 & 31.5 & 341.2 \\ 
        ~ &\cellcolor{Gray} SepLLM &\cellcolor{Gray} 800 &\cellcolor{Gray} 562 &\cellcolor{Gray} 28.3 &\cellcolor{Gray} 325.8 \\ \hline
        \multirow{3}{*}{64K} & Vanilla & 64K & 32K & 1090.8 & 3380.6 \\ 
        ~ & StrmLLM & 800 & 800 & 37.9 & 1096.0 \\ 
        ~ &\cellcolor{Gray} SepLLM &\cellcolor{Gray} 800 &\cellcolor{Gray} 562 &\cellcolor{Gray} 33.4 &\cellcolor{Gray} 1049.7 \\ 
    \end{tabular}
    \vspace{-2mm}
    \caption{The average perplexity and running time comparison on the PG19 test set~\cite{raecompressive2019}. \rKV~means the average \textit{runtime} KV cache usage in the generation process.}
    \label{tab:infer_time}
    \vspace{-2mm}
\end{table}

Those results demonstrate that our SepLLM can achieve lower perplexity with less wall-clock time as well as lower average runtime KV usage, especially for longer sequences, given the same max KV cache capacity $\textit{\textbf{c}}$.
\vspace{-0.5mm}
\subsection{Ablation Study}
\label{sec:ablation_study}
\vspace{-0.5mm}


    


\paragraph{Hyperparameters.} We conduct various ablation experiments specifically for long-input applications. This includes a detailed study of the impact of various hyperparameters across different text lengths (5K to 20K). The experimental results about \textbf{\textit{s}} and (\textbf{\textit{w}},\textbf{\textit{c}}) pair are illustrated in Table~\ref{tab:segcache_size} and Table~\ref{tab:window_size} respectively. The conclusions are as follows.


\begin{table}[t]
\centering
\small
    \setlength{\tabcolsep}{8pt}
    \renewcommand{\arraystretch}{1.2}
\begin{tabular}{c|ccccc}
        \textbf{\textit{s}}             & 5K                   & 10K                  & 15K                  & 20K                  & \rKV \\ \shline
32 & 13.11              & 11.31              & 8.74               & 8.79               & 292                  \\
48 & 13.03              & 11.26             & 8.70             & 8.76               & 300                  \\
64  & 13.01              & 11.17              & 8.67               & 8.72               & 308    
\end{tabular}
\vspace{-2mm}
\caption{The perplexity and average \textit{runtime} KV cache usage of SepLLM with respect to different Separator Cache capacities (\textit{\textbf{s}}) on WikiText~\cite{merity2016pointer}, in which \textit{\textbf{a}}=4, \textit{\textbf{w}}=224, \textit{\textbf{c}}=324.} 
\label{tab:segcache_size}
\vspace{-3.8mm}
\end{table}

\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{c|ccc|cccc}
Method &  \textbf{\textit{w}}   & \textbf{\textit{c}}   & \rKV & 5K      & 10K     & 15K    & 20K    \\ \shline
      & 320 & 324 & 324   & 13.18 & 11.51 & 8.85 & 8.91 \\
StrmLLM      & 512 & 516 & 516   & 12.87 & 11.37 & 8.74 & 8.78 \\
     & 796 & 800 & 800   & 11.96 & 11.01 & 8.67 & 8.72 \\ \hline\rowcolor{Gray}
    & 224 & 324 & 308   & 13.01 & 11.17 & 8.67 & 8.72 \\\rowcolor{Gray}
SepLLM    & 320 & 516 & 452   & 12.91 & 11.26 & 8.67 & 8.72 \\\rowcolor{Gray}
 & 512 & 800 & 690   & 12.09 & 11.03 & 8.56 & 8.62
\end{tabular}
\vspace{-3mm}
\caption{{Average downstream performance (ppl) over different input lengths and average \textit{runtime} KV usage with different \textit{\textbf{c}},\textit{\textbf{w}} on WikiText, in which \textit{\textbf{a}}=4 for both methods and \textit{\textbf{s}}=64 for SepLLM.}}
\label{tab:window_size}
\vspace{-1.9mm}
\end{table}


\begin{itemize}[leftmargin=*,nosep]
\setlength\itemsep{0.6em}
    \item  \textbf{\textit{s}}: From Table~\ref{tab:segcache_size}, the capacity of Separator Cache affects the perplexity of long-text inference, as we find that increasing \textit{\textbf{s}} leads to a certain degree of perplexity reduction.   
    \item  \textbf{\textit{c}} and \textbf{\textit{w}}:  As can be seen in Table~\ref{tab:window_size}, \textbf{\textit{c}} and \textbf{\textit{w}} can impact the average perplexity in the scenario of long streaming input with lengthy text. Moreover, as they increase, the perplexity decreases accordingly.  
\end{itemize}

\paragraph{Settings.} We also perform the following experiments to validate the effectiveness of Initial Tokens and Positional Encoding's shifting for both StreamingLLM and SepLLM. The experimental results are shown in Table~\ref{tab:abl_sink_shfit} and the discussions are as follows.


\begin{itemize}[leftmargin=*,nosep]
\setlength\itemsep{0.6em}
    \item  \textbf{Initial Tokens}: Initial Tokens are crucial for modeling context of long streaming inputs, whether for~\model~or StreamingLLM. Removing them has a significant impact on the perplexity of long texts. This conclusion is consistent with the paper~\cite{xiao2024efficient}.
    \item  \textbf{Positional Encoding's Shifting}. Following streamingLLM, we conduct Positional Shifting for streaming applications, \ie, we focus on positions within the cache rather than those in the original text. Table~\ref{tab:abl_sink_shfit} shows that this shifting plays a crucial role, as removing it significantly increases the perplexity (StreamingLLM increases from around 13 to over 400). It is noteworthy that~\model, even without employing this shifting, only sees a perplexity increase to around 200, which is much lower than StreamingLLM. This further underscores the separators' role for the stability in predicting tokens.
\end{itemize}





\paragraph{Separator Choices.} A series of ablation studies are also conducted on the choice of separators. For SepLLM, whether it is the \textit{Fundamental Design} or the \textit{Tailored Streaming Design}, the choice of separator types serves as a kind of hyperparameter. Given that the types of common separators are limited (\eg, the ones we adopt here [``.", ``,", ``?", ``!", ``;", ``:", `` ", ``\textbackslash t", ``\textbackslash n"]), we recommend including all commonly used ones. A detailed discussion of the ablation studies on separators is provided in Appendix~\ref{app:sep_choice}.


\begin{table}[!t]
\centering
\small
\setlength{\tabcolsep}{3.5pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lcc|ccccc}
Method & initial & shift & 5K       & 10K      & 15K      & 20K      & \rKV \\ \shline
StrmLLM   & \cmark    & \cmark     & 13.2  & 11.5  & 8.9   & 8.9   & 324  \\
StrmLLM   & \xmark    & \cmark     & 14.6  & 13.2  & 10.8  & 10.9  & 324  \\
StrmLLM   & \cmark    & \xmark     & 425.5 & 513.1 & 509.5 & 506.8 & 324  \\
StrmLLM   & \xmark    & \xmark     & 409.4 & 540.5 & 527.5 & 558.2 & 324  \\ \hline\rowcolor{Gray}
SepLLM   & \cmark    & \cmark     & 13.1  & 11.3  & 8.7   & 8.8   & 292  \\\rowcolor{Gray}
SepLLM   & \xmark    & \cmark     & 14.9  & 14.3  & 12.4  & 12.5  & 290  \\\rowcolor{Gray}
SepLLM   & \cmark    & \xmark     & 192.7 & 214.6 & 175.0 & 174.4 & 292  \\\rowcolor{Gray}
SepLLM   & \xmark    & \xmark     & 226.4 & 264.7 & 227.5 & 228.8 & 290 
\end{tabular}
\vspace{-2mm}
\caption{ The perplexity and average \textit{runtime} KV cache usage of SepLLM and StreamingLLM tested on WikiText~\cite{merity2016pointer}. \textit{\textbf{c}}=324, \textit{\textbf{a}}=0/4 for both methods. \textit{\textbf{s}}=32,\textit{\textbf{w}}=224 for SepLLM}.
\label{tab:abl_sink_shfit}
\vspace{-6mm}
\end{table}



\subsection{Comparison with More Baselines and Variants}
\paragraph{Naive Baseline.} We compare SepLLM with more baselines and variants to verify its effectiveness. The results shown in Table~\ref{tab:sparse_hd_cmp} are based on a naive baseline in which $H_s$ out of $H$ attention heads are configured as sliding window attention, while the remaining heads use full attention. We use MMLU as the benchmark to measure the differences in reasoning ability, ensuring that the runtime KV usage for all methods is kept as consistent as possible. It can be observed that this naive head-wise baseline performs poorly (regardless of how many full attention heads are retained), which is due to the heterogeneity among the heads. In contrast, SepLLM achieves performance very close to Vanilla across various knowledge domains with the same KV usage.
\paragraph{State-of-the-Art Baselines.} In addition, we compare SepLLM with multiple state-of-the-art baseline methods, which demonstrates the effectiveness and simplicity of SepLLM. For detailed results, please refer to the Appendix~\ref{app:more_cmp}.
\paragraph{Fixed-Interval Variant.} Furthermore, to demonstrate the compression and summarization effects of separators on the information within the segments they divide, we propose a fixed-interval variant, FixLLM. In FixLLM, instead of attending to separator tokens, it attends to one token at fixed intervals, except for the Initial Tokens' and Neighboring Tokens' sections. We find that SepLLM significantly outperforms FixLLM, which indicates that the compression and summarization capabilities of separators in SepLLM cannot be replaced by fixed-interval tokens. Please see the Appendix~\ref{sec:appendix_fix_int} for detailed results and discussions.





\subsection{Generalization and Information Retrieval}
To verify the generalization of~\model, we adapt~\model~to models of different architectures and scales. The results and discussions in Appendix~\ref{app:diff} can validate the generalization capability of our proposed~\model. 
Specifically, we adapt~\model~to different backbones including Pythia-6.9B, Pythia-12B~\cite{biderman2023pythia}, Llama-3-8B-Base/Instruct~\cite{dubey2024llama} and Falcon-40B~\cite{falcon40b}.
Moreover, we also conduct the \textit{Needle-in-a-Haystack}
experiment, which further demonstrates the compression capability of separator tokens for segment information. As illustrated in Appendix~\ref{sec:append_needle}, SepLLM can retrieve the needle in most scenarios. In comparison, StreamingLLM~\cite{xiao2024efficient} cannot complete this task. In addition, we provide comparisons of SepLLM with more baseline models regarding mathematical reasoning and logical analysis capabilities in the Appendix~\ref{app:more_cmp}. Furthermore, Appendices~\ref{app:dis} and~\ref{sec:appendix_fix_int} discuss in detail the effects and functions of separators from the perspective of implementation logic.



\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{0.7mm}
\setlength\extrarowheight{2.5pt}
\begin{tabular}{c|ccccc|cc}
 &
  \multicolumn{5}{c|}{MMLU} &
   &
   \\ \cline{2-6}
\multirow{-2}{*}{$H_s$/$H$} &
  humanity &
  social &
  stem &
  other &
  overall &
  \multirow{-2}{*}{\rKV~(\%)} &
  \multirow{-2}{*}{\pn} \\ \shline
20/32 &     23.93 & 23.07 & 24.42 & 23.53 & 23.76 & 44.74 & 80 \\
24/32 &     24.23 & 23.30 & 26.36 & 23.37 & 24.31 & 47.71 & 208 \\
28/32 &     25.66 & 27.29 & 26.31 & 23.69 & 25.81 & 45.13 & 256 \\
30/32 &     27.29 & 25.09 & 27.78 & 38.11 & 29.31 & 45.42 & 288 \\ \hline \rowcolor{Gray}
SepLLM &    57.66 & 76.21 & 56.49 & 72.19 & 64.68 & 44.61 & 256 \\\rowcolor{Gray}
Vanilla &   60.49 & 76.50 & 56.61 & 72.19 & 65.72 & 100.00 & ALL
\end{tabular}
\caption{Comparison with a naive baseline method, where $H_s$ out of $H$  attention heads are set to sliding window attention, and the remaining heads use full attention. \pn~represents the number of Neighboring Tokens (\ie, the sliding window size). \rKV~(\%) indicates the ratio of KV usage at \textit{runtime} for the respective method compared to Vanilla.}
\label{tab:sparse_hd_cmp}
\end{table}




































\section{Universal Approximation} %

In this section, we present the theoretical results on the universal approximation capabilities of encoder-based SepLLM. Details can be found in Appendices~\ref{sec:appendix_uni_appr} and~\ref{sec:appendix_proof4appr}.



Let $\mathcal{T}_{\text{Sep}}^{H,d_h,d_f}$ be the class of SepLLM, where $H$, $d_h$, and $d_f$ represent the number of heads, hidden dimension in attention layers, and the hidden dimension of feed-forward layers, respectively. 
Denote $\mathcal{F}$ as the class of continuous functions $f: [0,1]^{d \times n} \to \mathbb{R}^{d \times n}$, where $d$ and $n$ represent the dimensionality of input tokens and the sequence length, respectively. For any $p\geq 1$, we use the $\ell_{p}$ distance to measure the difference between two continuous functions $f_1, f_2 \in \mathcal{F}$, defined as $\left(\int_{[0,1]^{d \times n}} \left\|f_1(\bm{X}) - f_2(\bm{X}) \right\|_{p}^{p} d \bm{X} \right)^{1/p}$. The following theorem shows that the proposed SepLLM holds the universal approximation to arbitrarily sequence-to-sequence continuous functions. For the complete proof and derivation process, please refer to the Appendices~\ref{sec:appendix_uni_appr} and~\ref{sec:appendix_proof4appr}.

\begin{theorem}
    Given $p>1$ and $n>2$, for any $\epsilon>0$ and $f \in \mathcal{F}$, there exists a SepLLM $g \in \mathcal{T}_{\text{Sep}}^{2,1,4}$, such that $d_{p}\left(f,g \right) < \epsilon$.
\end{theorem}


==> spjvjgywrcgsfttxpzygsccdcktfvmxn_arXiv/latex/intro.tex <==
\vspace{-5mm}
\section{Introduction}
\label{sec:intro}
\vspace{-.5mm}

\begin{figure}[t]
\centering
\includegraphics[width=0.49\linewidth]{fig/TFLOPs_ext3_SepLLM_v5.pdf}
\includegraphics[width=0.495\linewidth]{fig/training_loss_time_sim3_SepLLM_v5.pdf}
\vspace{-8mm}
\caption{The loss comparison between vanilla Transformer and the proposed SepLLM. SepLLM achieves lower loss \wrt~different computation costs and different training time consistently.}
\label{fig:TFLOPs}
\vspace{-3mm}
\end{figure}

Transformer-based models \citep{NIPS2017_transformer} have exhibited exceptional performance across a wide range of tasks, including natural language processing \citep{zhang2020pegasus,raffel2020exploring}, computer vision \citep{dosovitskiy2020image}, and scientific machine learning \citep{geneva2022transformers}. 
However, vanilla Transformers that rely on next-token prediction face significant computational challenges, particularly when scaling to larger models and longer contexts. These computational inefficiencies significantly impact both inference speed and training time.


The core challenge underlying these efficiency issues is the self-attention module, which exhibits quadratic complexity with respect to the number of input tokens. Research on efficient Transformers in LLMs primarily follows two major directions.
The first approach focuses on linear attention~\citep{katharopoulos2020transformers,schlag2021linear}, replacing the vanilla self-attention module with alternatives that achieve linear complexity. %
However, these modifications make the architecture significantly different from traditional self-attention, preventing direct utilization of powerful pre-trained Transformer models. The second approach emphasizes KV cache optimization \cite{xiao2024infllm,zhu2024sampleattention,xiao2024efficient,li2024snapkv}, aiming to eliminate redundant KV cache to accommodate longer input contexts.
For example, \citet{xiao2024infllm} introduced an adaptive mechanism that selectively retains essential tokens and their KV based on cumulative attention scores. 
Similarly, \citet{zhu2024sampleattention} proposed a token selection strategy with controlled sparsity, achieving near-lossless acceleration. 
While promising, these training-free methods adapt poorly to the training stage, resulting in discrepancies between training and inference performance.
StreamingLLM~\citep{xiao2024efficient} represents a notable attempt to address these limitations by preserving attention sinks and local tokens to reduce computation and memory overhead. %
However, it omits many intermediate tokens, resulting in performance degradation compared to standard Transformers.



\begin{figure}[t]
    \centering
    \includegraphics[width=0.333\linewidth]{fig/a1.png}
    \includegraphics[width=0.32\linewidth]{fig/a2.png}
    \includegraphics[width=0.318\linewidth]{fig/a3.png}
    \vspace{-5mm}
    \caption{The visualization for attention scores of different layers given the input ``Natalia sold clips to 48 of her friends in April, and then she sold half as many clips in May. ...''. Note that the separator tokens like ``,'' and ``.'' contribute massive attentions.}    
    \vspace{-3mm}
    \label{fig:special_tokens}
\end{figure}






To gain better understanding of the intrinsic mechanism of LLMs, we analyze attention patterns across different samples. Figure~\ref{fig:special_tokens} illustrates the attention distribution when Llama-3-8B-instruct~\cite{dubey2024llama} processes a math problem (complete results are presented in Appendix~\ref{app:vis_attn}).     
Surprisingly, rather than focusing on semantically meaningful tokens (such as nouns and verbs), LLMs tend to prioritize attention to seemingly ``meaningless" separator tokens (like ``.'' or ``$\backslash n$'') for information retrieval.
This observation suggests that segment information is compressed and embedded into these separator tokens, enabling efficient information retrieval without direct extraction from content tokens.

Inspired by this observation, we introduce SepLLM, a new language modeling perspective as well as an efficient transformer architecture featuring a data-dependent sparse attention mechanism that selectively retains only initial, neighboring, and separator tokens while dropping other tokens. The training-free SepLLM performs comparably to vanilla Transformer, which validates our hypothesis that segment information is effectively compressed into separator tokens.
More importantly, we integrate SepLLM into the training stage (including both training from scratch or finetuning) and implement a hardware-efficient kernel based on FlexAttention~\cite{flexattn}. This integration reduces the discrepancies between training and inference that are present in previous approaches. 
As demonstrated in Figure~\ref{fig:TFLOPs}, SepLLM consistently achieves lower loss compared to vanilla Transformer given the same computational costs or training time.
Moreover, SepLLM reduces computational costs by 28\% and training time by 26\% while achieving the same training loss. Our contributions are summarized as follows:

\begin{itemize}[leftmargin=*,nosep]
\setlength\itemsep{0.5em}
\item We analyze attention patterns by visualizing token-level attention scores, revealing that initial, neighboring, and separator tokens consistently receive high attention weights. Such empirical findings motivate us to propose SepLLM, \textbf{a new language modeling perspective} and a simple yet effective framework to accelerate inference.
\item Through targeted masking experiments on well-trained LLMs, we demonstrate that separator tokens contain crucial information and are essential for model performance. This finding suggests that sequences are initially segmented by separators, with segment information being compressed into these frequently-attended separator tokens while redundant specific tokens can be discarded.
\item We conduct comprehensive experiments to validate SepLLM's effectiveness across various tasks, datasets, and backbone models, examining performance in training-free, training-from-scratch, and post-training settings.
\item We have made our implementation publicly available at \href{https://sepllm.github.io/}{\textbf{sepllm.github.io}}. Our codebase supports efficient multi-node distributed training with accelerated attention module \textit{Sep-Attention} and also supports numerous existing Fusion Operators to accelerate the training process, such as \textit{fused rope}~\cite{su2024roformer}, \textit{fused layer norm}, etc.
\end{itemize}




==> spjvjgywrcgsfttxpzygsccdcktfvmxn_arXiv/latex/method.tex <==
\vspace{-.9mm}
\section{Method}
\label{sec:method}
\subsection{Fundamental Design}
\label{sec:funda_design}
From Figure~\ref{fig:special_tokens}, we can observe that within a given input context, seemingly ``meaningless" separator tokens receive higher attention scores compared to tokens with actual semantic meanings. Therefore, we propose a novel Transformer architecture where, for a certain layer of the Transformer (\ie, a self-attention layer), each token in the input can only see a portion (not all) of the hidden states of tokens preceding the current token, outputted by the previous transformer layer. This subset of tokens includes a number of initial words (\eg, attention sinks~\cite{xiao2024efficient}), all the separator tokens before the current token, and the closest $\textit{\textbf{n}}$ tokens to the current token. Details are as follows.

\textbf{Initial Tokens}.
    When using the sliding window mechanism ~\cite{beltagy2020longformer} for generation, removing the key-value (KV) pairs corresponding to the initial tokens in the KV cache results in a noticeable increase in the perplexity of generated tokens, a phenomenon mentioned by ~\citet{xiao2024efficient}. The initial few tokens are also referred to as attention sinks. We retain this setup and further validate the role of initial tokens in subsequent experiments. Usually, $\textbf{\textit{a}}$ initial tokens are kept. 

    \textbf{Separator Tokens}. From Figure~\ref{fig:special_tokens}, we can observe that within a given input context, seemingly ``meaningless" separator tokens (such as commas, periods, exclamation marks, semicolons, etc.) that segment sequences receive higher attention scores compared to semantically meaningful tokens (such as nouns or verbs). Therefore, we hypothesize that these separators may compress the information of the text segments naturally segmented by them, such that when the Transformer generates new tokens, it only needs to reference the information contained in these separators to extract the information pertaining to those text segments. Hence, in a training-free scenario, we employed this strategy and achieved similar results to the original model based on full attention across many tasks. Furthermore, to reinforce the effect of using separators to compress information within their respective segments, we employed training-from-scratch and post-training approaches to compel the model during training to restrict the current token from accessing all information from distant preceding text, \ie, in each segment, only the separator representing its segment is visible to the current token (with other tokens being masked, see Figure~\ref{fig:pre-fill_gen_mask}).
    After training in this manner, the information within segments is forced to be condensed into the separators, leading the Transformer's probability distribution for predicting the next word closely resembling that of the original Transformer with full attention. See more in Appendices~\ref{app:dis} and~\ref{sec:appendix_fix_int}.
    
    \textbf{Neighboring Tokens}. Language tasks usually exhibit strong local dependencies and interactions, since adjacent tokens often form coherent phrases or have dependencies that are required to be captured. Neighboring tokens usually help form locally smooth and coherent contexts, allowing the model to generate sentences that are reasonable within the immediate context. The neighboring tokens, also referred to as local attention or sliding-window attention, are considered in various efficient Transformers \citep{xiao2024efficient,zhang2024h2o} and we have also adopted this approach, with the number of preceding tokens closest to the current token denoted as ``$\textit{\textbf{n}}$".    


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{fig/figure3.pdf}
    \vspace{-0.2in}
    \caption{The overall paradigm of~\model . The left side illustrates the attention mask in the training or pre-filling stage given the input ``ABC{$,$}DE{$.$}FG{$\backslash n$}". The right side illustrates the KV cache management in the generation stage.}
    \label{fig:pre-fill_gen_mask}
\end{figure}


\begin{figure*}[t]
    \begin{center}
    \includegraphics[width=0.99\linewidth]{fig/figure4_mod.pdf}
    \end{center}
    \vspace{-0.18in}
    \caption{Overall framework of the proposed \model\ tailored for streaming applications. The KV pairs are storaged in four cache blocks (displayed as four columns), and are updated in each iteration (shown in a single row). Once the runtime usage $Size_{run}$ reach the max capacity $\textbf{c}$, SepLLM move KV caches of separator tokens in Past Window Cache into Separator Cache and drop other KV caches.}
    \label{fig:streaming_design}
    \vspace{-0.1in}
\end{figure*}

\subsection{Overall Pipeline}
We split the overall pipeline of our proposed SepLLM into training/pre-filling stage and generating stage. We also provide a theoretical analysis about the \textit{Universal Approximation} of~\model~in Appendices~\ref{sec:appendix_uni_appr} and~\ref{sec:appendix_proof4appr}.

\paragraph{Training/Pre-filling.} During the training/pre-filling stage of ~\model~ architecture, we do not need to multiply all query vectors corresponding to tokens in the input context with all the key vectors. It is sufficient to just multiply the vectors of the query-key pairs corresponding to the highlighted elements in the mask matrix shown in Figure~\ref{fig:pre-fill_gen_mask}. The formulation can be illustrated in the following.
\begin{align}
\A\! = \!\text{Softmax} \left(   \Lambda  \right),\Lambda \!= \!\frac{  \text{Mul} \left( \Q,~\K^{\top} \big| ~\M  \right)  }{ \sqrt{d_k}   }\vspace{-0.6in} \!\!\notag  \\
\O = \A \cdot \V~~~~~~~~~~~~~~~~~~~~~~~~~~
\label{eq:pre-fill_atten}
\end{align}
where $\Q \in \domR^{m \times d_k},\K \in \domR^{m \times d_k}$ are the matrices of query and key for one attention layer, in which each row vector $\Q_{i},\K_{j}$ correspond to the query of $i$-th token and the key of $j$-th token in the input context with sequence length $m$. $d_k$ denotes the dimension for key and query vectors. ${\Lambda}, \A \in \domR^{m \times m}$ are the raw and final attention maps, respectively. $\V \in \domR^{m \times d_v}$ is value matrix of dimension $d_v$ and $\O \in \domR^{m \times d_v}$ denotes the output for the current attention layer. $\text{Mul}(\cdot)$ represents a sparse matrix multiplication function which can be optimized by methods like~\citet{zhu2024sampleattention} and we also implement our own module named \textit{Sep-Attention} to accelerate this process. $\M \in \domB^{m \times m}$ is a binary mask matrix\!\footnote{$\domB\coloneqq\{0,1\}$, which is a binary set.} used as a parameter for $\text{Mul}(\cdot)$:
\begin{equation}
{\Lambda}_{i,j}  =\left\{
\begin{aligned}
\Q_{i}^{\top}\K_{j} / \sqrt{d_k}~, ~~& \text{if}~~\M_{i,j}=1 \\
-\infty~, ~~~~~~~~& \text{if}~~\M_{i,j}=0  \\
\end{aligned}
\right..
\end{equation}
where $\Lambda_{i,j},\A_{i,j},\M_{i,j}$ are the elements in the $i$-th row and $j$-th column of matrices $\Lambda,\A,\M$, respectively. 
Since ${\A_{i,j}}=0$ if ${\Lambda_{i,j}}=-\infty$, the tokens that are not \textit{Initial}, \textit{Separator}, and \textit{Neighboring} tokens will be masked by $\A \cdot \V$ in Equation~\ref{eq:pre-fill_atten}. This strategy (Equation~\ref{eq:pre-fill_atten}) applies to all heads of multi-head attention~\citep{NIPS2017_transformer}.



\paragraph{Generation.} The management of the KV cache during the generation stage for this \textit{Fundamental Design} (Section~\ref{sec:funda_design}) is also intuitive. 
As shown in the right side of Figure~\ref{fig:pre-fill_gen_mask}, when generating a new token, we only preserve the KV cache for the \textit{Initial}, \textit{Separator}, and \textit{Neighboring} tokens. Therefore, the KV cache in the proposed SepLLM is much smaller and requires less memory.
Ideally, based on~\model, the perplexity of generating the next word is comparable to that of the original Transformer with full attention.




\subsection{Tailored Streaming Design}
\label{sec:stream_design}
In real-world scenarios, there are numerous streaming applications such as multi-round dialogues, where long interactions are expected~\citep{xiao2024efficient}. Hence, we expect SepLLM to handle infinite input without significantly sacrificing efficiency and performance, especially for streaming applications. As discussed in \textit{Fundamental design} (Section~\ref{sec:funda_design}),  SepLLM can save a substantial amount of KV cache by retaining only the KV for separator, neighboring, and initial tokens. However, as the number of input tokens increases, the number of separators in KV cache will also accumulate endlessly, which is not feasible for streaming settings. Therefore, we propose \textit{Tailored Streaming Design} for streaming scenarios.
\paragraph{Framework.} Figure~\ref{fig:streaming_design} illustrates the~\model's processing architecture for streaming applications. The diagram depicts multiple iterations, with each row representing a distinct processing step. The system simultaneously maintains four specialized cache blocks: Initial Cache, Separator Cache, Past Window Cache, and Local Window Cache.
Specifically, Initial Cache captures the attention sinks proposed by \citet{xiao2024efficient}. Local Window and Past Window Caches store the KV  for consecutive tokens, with Past Window Cache serving as an overflow buffer for the Local Window Cache. Separator Cache retains the KV  for separators which contain condensed segment information. 

To describe the cache management strategies, we denote the runtime usage of the four caches as $Size_{\text{init}}$, $Size_{\text{sep}}$, $Size_{\text{past\_w}}$, and $Size_{\text{local\_w}}$, respectively. The runtime usage across all KV caches is defined as $Size_{\text{run}} \coloneqq Size_{\text{init}}+Size_{\text{sep}}+Size_{\text{past\_w}}+Size_{\text{local\_w}}$, which satisfies $Size_{\text{run}} \le \textbf{\textit{c}}$. The number of continuous Neighboring tokens is defined as $\textbf{\textit{n}}\!\coloneqq\!Size_{\text{past\_w}}\!+\!Size_{\text{local\_w}}$. Notably, \textbf{\textit{n}} is a function of the input sequence length $m$ (together with the specific input dataset $\mathcal{D}$) rather than a fixed hyperparameter for streaming setting.
For clarity, we detail the preset hyperparameters of this caching system as follows (\textit{Note}: $\textbf{\textit{a}}+\textbf{\textit{s}}+\textbf{\textit{w}}< \textit{\textbf{c}}$).
\vspace{-0.1in}
\begin{itemize}
    \item  \textbf{\textit{c}}: The maximum capacity of the entire KV cache.
    \vspace{-0.08in}
    \item  \textbf{\textit{a}}: The maximum capacity of Initial Cache.
    \vspace{-0.08in}
     \item  \textbf{\textit{s}}: The maximum capacity of Separator Cache. 
     \vspace{-0.08in}
    \item  \textbf{\textit{w}}: The maximum capacity of Local Window Cache. Notably, \textbf{\textit{w}} is also the minimum value of $\textbf{\textit{n}}$ after runtime KV cache usage $Size_{\text{run}}$ reaches $\textbf{\textit{c}}$ for the first time.
\end{itemize}



During streaming sequence generation, SepLLM will firstly fill Initial Cache and then Local Window Cache. After $Size_{\text{local\_w}}$ reaches $\textbf{\textit{w}}$, subsequent tokens are directed to Past Window Cache. Compression is triggered when $Size_{\text{run}}$ reaches $\textbf{\textit{c}}$ (iteration 1 in Figure~\ref{fig:streaming_design}), where separator tokens in Past Window Cache are moved to Separator Cache and other tokens are discarded.
When Separator Cache reaches its capacity $\textbf{\textit{s}}$ at some total input length $m_0$, $\textbf{\textit{n}}$ enters a periodic pattern. Specifically, for $m>m_0$, $\textbf{\textit{n}}$ follows a periodically linear function bounded by $\textbf{\textit{w}}$ and $\textbf{\textit{c}}-\textbf{\textit{a}}-\textbf{\textit{s}}$. The detailed evolution of KV caches is illustrated in Appendix~\ref{app:curve}. To analyze the average usage of KV cache, we define $\bar{\textbf{\textit{n}}}_m\coloneqq \frac{1}{m}\sum_{k=1}^m \textbf{\textit{n}}(k)$. According to the linearity and periodicity, we have
\begin{equation}
    \lim\limits_{m \to \infty}\!\bar{\textit{\textbf{n}}}_m  = \frac{  \textbf{\textit{w}} + \textbf{\textit{c}}-\textbf{\textit{a}}-\textbf{\textit{s}}  }{2}.
\end{equation}
For the average runtime KV cache usage of infinite-length sequence generation, we have
\begin{align}
\lim\limits_{m \to \infty}\!\overline{{Size}_{\text{run}}} &= \lim\limits_{m \to \infty}\! \bar{\textit{\textbf{n}}}_m + \textbf{\textit{a}}+\textbf{\textit{s}} \nonumber \\
&=\frac{  \textbf{\textit{w}} + \textbf{\textit{c}}+\textbf{\textit{a}}+\textbf{\textit{s}} }{2} < \textbf{\textit{c}}.
\end{align}

\paragraph{Positional Encoding.} Our positional encoding strategy for streaming settings is the same as the state-of-the-art StreamingLLM~\cite{xiao2024efficient}, designed specifically for infinite-length inputs, where we focus on positions within the cache instead of those in the original text. 








==> spjvjgywrcgsfttxpzygsccdcktfvmxn_arXiv/latex/related_work.tex <==
\vspace{-1mm}
\section{Related Work}
\vspace{-0.25em}
\label{sec:related_work}

\textbf{KV Cache Compression}. Recent research has focused on overcoming LLMs' limitations in processing extensive contextual inputs. FastGen \citep{ge2023model} proposes an adaptive KV cache management method, optimizing memory usage by customizing retention strategies for different attention heads. SnapKV \citep{li2024snapkv} enhances efficiency through KV cache compression, utilizing attention scores to select and cluster significant positions. H$_2$O~\citep{zhang2024h2o} implements a dynamic token retention policy, balancing recent and historically important information to optimize memory use. StreamingLLM \citep{xiao2024efficient} expands LLMs' capabilities to handle infinite sequence lengths without fine-tuning, by reserving attention sinks and local tokens. 
QuickLLaMA~\cite{li2024quickllama} proposes to evict the query-aware KV cache for inference acceleration.
PyramidInfer~\cite{yang2024pyramidinfer} and PyramidKV \citep{zhang2024pyramidkv} modify the KV cache capacity across different layers, prioritizing larger allocations in the lower layers while reducing those in the upper layers. However, most works in this category cannot be applied into training phase.%

\textbf{Sparse Attention}. Sparse attention involves creating sparse attention matrices by limiting attention to predefined patterns, such as local windows or fixed-stride block patterns. \citet{beltagy2020longformer} combine dilated local window attention with task-specific global attention. BigBird \citep{zaheer2020big} proposes a linear-complexity attention alternative using global tokens, local sliding-window attention, and random attention. In comparison, SparseBERT \citep{shi2021sparsebert} proposes a differentiable attention mask algorithm to learn the attention mask in an end-to-end manner. Note that most works about sparse attention are using fixed masks and built on BERT \citep{devlin2018bert} families. In comparison, our proposed SepLLM is mainly built on GPT~\cite{brown2020language} series and its attention masks are data-dependent. 

